Proximity-Induced Skyrmion Stabilization at the Cu2OSeO3/Bi2Se3 Interface

We investigate proximity-induced magnetic interactions at the interface between the topological insulator Bi2Se3 and the chiral magnetic insulator Cu2OSeO3, with particular focus on the low temperature skyrmion phase. Broadband ferromagnetic resonance spectroscopy reveals enhanced stability of noncollinear spin textures in the Cu2OSeO3/Bi2Se3 heterostructure compared with bare Cu2OSeO3. In addition to an extra resonance mode in the tilted conical phase that is absent in bare Cu2OSeO3, field cycling resolves two counterclockwise skyrmion resonance branches separated by approximately 238 MHz, consistent with the coexistence of a bulk skyrmion lattice and an interfacial skyrmion phase stabilized by proximity-induced exchange coupling and enhanced interfacial Dzyaloshinskii-Moriya interactions. The finite frequency separation indicates that the two skyrmion phases occupy distinct magnetic energy landscapes while retaining similar resonance character. Resonant elastic x-ray scattering measurements further confirm that the interfacial skyrmion phase spans a broader magnetic-field range than the bulk phase, demonstrating enhanced stability and ordering of topological spin textures at the interface. These findings establish interface engineering as a promising route for extending the stability regime of skyrmion and tilted-conical phases in topological-magnetic heterostructures.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{romannum}
\usepackage{tikz}
\usepackage{miller}
\usepackage{romannum}
\usepackage{float}
\usepackage{placeins}
\usepackage{svg}
\usepackage{layouts}
\usepackage{printlen}
% \newcommand{\cso}{Cu$_2$OSeO$_3$}
% \newcommand{\CSO}{Cu$_2$OSeO$_3$ }
% \newcommand{\CSOBS}{Cu$_2$OSeO$_3$/Bi$_2$Se$_3$ }
% \newcommand{\csobs}{Cu$_2$OSeO$_3$/Bi$_2$Se$_3$}
% \newcommand{\bss}{Bi$_2$Se$_3$}
% \newcommand{\BS}{Bi$_2$Se$_3$ }

\newcommand{\cso}{CSO}
\newcommand{\CSO}{CSO }
\newcommand{\CSOBS}{CSO/BS }
\newcommand{\csobs}{CSO/BS}
\newcommand{\bss}{BS}
\newcommand{\BS}{BS }
